Expressive Power of Temporal Message Passing

Graph neural networks (GNNs) have recently been adapted to temporal settings, often employing temporal versions of the message-passing mechanism known from GNNs. We divide temporal message passing mechanisms from literature into two main types: global and local, and establish Weisfeiler-Leman characterisations for both. This allows us to formally analyse expressive power of temporal message-passing models. We show that global and local temporal message-passing mechanisms have incomparable expressive power when applied to arbitrary temporal graphs. However, the local mechanism is strictly more expressive than the global mechanism when applied to colour-persistent temporal graphs, whose node colours are initially the same in all time points. Our theoretical findings are supported by experimental evidence, underlining practical implications of our analysis.

==> types.tex <==

\section{Types of Temporal Message Passing}

In this section, we will 
identify and formalise  types of temporal message passing mechanisms used in \TGNN{}s.
As a result, we will obtain four main types, which we will analyse from the theoretical and experimental points of view in the upcoming sections.

We start by providing a general form of a message-passing \TGNN{} model $\model$ with $L$ layers.
Given a temporal graph $\TG = (\G_1,t_1), \dots, (\G_n,t_n)$, it computes for each node $v$, each time point $t$, and  each layer $\ell \in \{0,\ldots,L\}$
an embedding $\h_v^{(\ell)}(t)$ as follows:
\pw{(3) mentions function $g$, but we never used different $g$. We can maybe say that $g(t-t')=t-t'$ gives highest expressiveness? Or maybe $g$ does not impact our results at all? It should be checked properly.}
\begin{align}
\h_v^{(0)}(t) &= \x_v(t), \label{TGN1}
\\
\h_v^{(\ell)}(t) &= \com^{(\ell)} \Big(
\h_v^{(\ell-1)}(t),
\agg^{(\ell)}(
\label{TGN2}
\\ 
& \ldblbrace
( \fone, g(t-t') ) \mid
 (u,t') \in \NH_{\TG}(v,t) 
\rdblbrace
)
\Big), \nonumber
\end{align}
where:
\begin{itemize}
\item $\com^{(\ell)}$ and $\agg^{(\ell)}$ are \emph{combination} and \emph{aggregation} functions in layer $\ell$; a combination function maps a pair of vectors into a single vector, whereas an aggregation function maps a multiset into a single vector,
\item $\fone$ is  $\mathbf{h}_u^{(\ell-1)}(t')$ or $\mathbf{h}_u^{(\ell-1)}(t)$, depending on the type of the message passing mechanism,
\item $g$ maps a time distance between two time points into a single value (e.g. into a vector),
\item $\NH_{\TG}(v,t)$ is the temporal neighbourhood of $(v,t)$, as defined in Equation~\eqref{eq:NH}.
\end{itemize}
Hence, the extension of the standard message passing consists in modifying the aggregation mechanism, which now (i)~aggregates over the temporal neighbourhood $\NH_{\TG}(v,t)$, (ii)~aggregates either embeddings $\mathbf{h}_u^{(\ell-1)}(t')$ or $\mathbf{h}_u^{(\ell-1)}(t)$, and (iii)~uses the time distance $t-t'$ in the aggregation process.

The main difference between \TGNN{} models introduced in the literature is the form $\fone$ of the embeddings which are aggregated.
In particular, the class of \emph{Temporal Embedding} \TGNN{}s~\cite{longa2023graph}, which include such models as TGAT~\cite{DBLP:conf/iclr/XuRKKA20} and NAT~\cite{DBLP:conf/log/LuoL22}, aggregate embeddings  $\mathbf{h}_u^{(\ell-1)}(t')$ for each temporal neighbour $(u,t')$. 
For example, to compute $\h_a(t_4)$ for $\TG$ from \Cref{fig:snapshot}, a model would aggregate $\h_c(t_4)$ and $\h_b(t_2)$.
On the other hand, models such as  TGN~\cite{DBLP:journals/corr/abs-2006-10637} and TDGNN~\cite{DBLP:conf/www/QuZDS20}, to compute an embedding of $(v,t)$ aggregate embeddings of  $\mathbf{h}_u^{(\ell-1)}(t)$ for all temporal neighbours $(u,t')$ of $(v,t)$.
In other words, messages are  passed not from temporal neighbours $(u,t')$, but from their ``future counterparts'' $(u,t)$ at $t \geq t'$. 
As a result, to compute embeddings at $t$ it is not necessary to keep in memory embeddings in other time points.
For example, to compute $\h_a(t_4)$ for $\TG$ from \Cref{fig:snapshot}, a model would aggregate $\h_c(t_4)$ and $\h_b(t_4)$.
The seemingly minor difference between using $\mathbf{h}_u^{(\ell-1)}(t')$ or $\mathbf{h}_u^{(\ell-1)}(t)$ in Equation~\eqref{TGN2}, as we will show in the paper, has a significant impact on the temporal message passing mechanism and on the expressive power of resulting \TGNN{}.

The second distinction we will consider, is on the form of temporal graphs taken as inputs by \TGNN{}s.
Some models, like TGAT, NAT, and TGN, apply temporal message passing to temporal graphs given in the snapshot representation (or in the event-based representation which can be transformed into the snapshot representation), whereas other models, such as TDGNN, 
take as an input an aggregated representation.
Recall that the aggregated representation can be transformed into the snapshot representation (see \Cref{fig:aggregated}), but not vice versa.
Hence, allowing for input temporal graphs only in the aggregated representation potentially restricts the expressive power of a model.

Depending on the form of $\fone$ and on the assumed representation of the input temporal graph, we obtain four types of temporal message passing models, as presented in
\Cref{tab:types}.
In what follows, we will show how the expressive power of a model depends on these choices.
As the main tool for establishing expressive power results, we will use a Weisfeiler-Leman characterisation for \TGNN{}s which we provide in the next section.

% the differences and similarities between three message passing mechanisms identified in the previous section, namely for MP-TGN in Equations   \eqref{TGN1}--\eqref{TGN2}, for  TA in Equations   \eqref{TE1}--\eqref{TE2}, and for 
% TD in Equations \eqref{TD1}--\eqref{TD2}.
% These three types of message passing differ in the definition of the definition of the initial embeddings $\h_v^{(0)}(t)$, which can be either $\x_v(t)$ or $\x_v$, and in the definition of embeddings $\mathbf{h}_u^{(\ell-1)}$ used withing the aggregation function, which can be either $\mathbf{h}_u^{(\ell-1)}(t)$ or $\mathbf{h}_u^{(\ell-1)}(t')$ (where $t'$ is the time point in which there was an edge from $u$).
% \Cref{tab:comp} summarises how the impact of these choices on the type of message passing mechanism.
% To complete the landscape of temporal message passing mechanisms we include in the table also a new type \new{}, which uses the same feature vectors across the time (like TDGNN) and aggregates embeddings from time points $t'$ (as TE).

% \begin{definition}
% A message passing \TGNN{} is a tuple $\model = ( L, \{  \agg^{(\ell)} \}_{\ell=1}^L , \{\com^{(\ell)} \}_{\ell=1}^L , \fone, \ftwo, g )$ where:
% \begin{itemize}
% \item $L \in \N$ is the number of layers,
% \item $\agg^{(\ell)}: \Box^{\R^d} \to \R^d$ is an aggregation function (where $\Box^{\R^d}$ is the set of all multisets which have $\R^d$
%  as their support set),
% \item $\com^{(\ell)}: \R^d \times \R^d \to \R^d$ is a composition function,
% \item $\fone(v)$ is $\x_v(t)$ or $\x_v$,
% \item $\ftwo$ is $\mathbf{h}_u^{(\ell-1)}(t)$ or
%  $\mathbf{h}_u^{(\ell-1)}(t')$,
% \item $g: \R \to \R^d$,
% \end{itemize}

% Finally each $v$ at $t$ is classified as $\cls(\h_v^{(L)}(t)) \in \{\true , \false \}$, denoted as $\model(\TG,v,t)$.
% \end{definition}


\pwline{I do not like the distinction between T1-T4. 

Maybe Give some names to T1 and T2, say global and local message passing, respectively?

Then, instead of T3 and T4 have  coloured vs uniformly coloured graphs?}

\begin{table}[ht]
\centering
\begin{tabular}{cc|cc|c}
                                            &    & \multicolumn{2}{c|}{Input temporal graph:}                  &  \\ %\cline{3-4}
                                            &    & \multicolumn{1}{l|}{snapshot} & aggregated &  \\ \cline{1-4}
\multicolumn{1}{c}{\multirow{2}{*}{$\fone=$}} & $\mathbf{h}_u^{(\ell-1)}(t')$  & \multicolumn{1}{c|}{\Tone{}}        &      \Tthree{}      &  \\ \cline{2-4}
\multicolumn{1}{c}{}                      & $\mathbf{h}_u^{(\ell-1)}(t)$ & \multicolumn{1}{c|}{\Ttwo{}}         &     \Tfour{}        &  \\ \cline{1-4}
\end{tabular}
\caption{Types of $\TGNN{}$s}
\label{tab:types}
\end{table}


